DP2Guard: A Lightweight and Byzantine-Robust Privacy-Preserving Federated Learning Scheme for Industrial IoT

Privacy-Preserving Federated Learning (PPFL) has emerged as a secure distributed Machine Learning (ML) paradigm that aggregates locally trained gradients without exposing raw data. To defend against model poisoning threats, several robustness-enhanced PPFL schemes have been proposed by integrating anomaly detection. Nevertheless, they still face two major challenges: (1) the reliance on heavyweight encryption techniques results in substantial communication and computation overhead; and (2) single-strategy defense mechanisms often fail to provide sufficient robustness against adaptive adversaries. To overcome these challenges, we propose DP2Guard, a lightweight PPFL framework that enhances both privacy and robustness. DP2Guard leverages a lightweight gradient masking mechanism to replace costly cryptographic operations while ensuring the privacy of local gradients. A hybrid defense strategy is proposed, which extracts gradient features using singular value decomposition and cosine similarity, and applies a clustering algorithm to effectively identify malicious gradients. Additionally, DP2Guard adopts a trust score-based adaptive aggregation scheme that adjusts client weights according to historical behavior, while blockchain records aggregated results and trust scores to ensure tamper-proof and auditable training. Extensive experiments conducted on two public datasets demonstrate that DP2Guard effectively defends against four advanced poisoning attacks while ensuring privacy with reduced communication and computation costs.

==> cover_letter.tex <==
\pagestyle{empty}
\pagenumbering{gobble}

% \onecolumn
% \centerline{\textbf{\huge Response to Reviewers' Comments}}
% \vspace{2mm}
\setcounter{page}{1}

\newboolean{showquestion}
\setboolean{showquestion}{true}
% \setboolean{showquestion}{false}

% Disable automatic numbering for figures and tables in cover letter only
% This ensures cover letter numbering doesn't affect manuscript.tex
\captionsetup[figure]{labelformat=empty}
\captionsetup[table]{labelformat=empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent \textbf{Summary of Revisions} 
% \vspace{2mm}

% \noindent
\noindent \textbf{[Paper \#TMC-2025-07-2021] Response to Reviewers’ Comments.}
We would like to thank the editor and reviewers for their constructive comments. 
We have addressed all the comments in the revised version.
To facilitate review, the major revisions associated with the \revmeta{Associate Editor}, \revone{Reviewer 1} and \revtwo{Reviewer 2} are highlighted in their respective colors. 
In the following, we first summarize the major changes and then provide detailed point-by-point responses to all reviewer comments.
Here, \revone{R1.Cx} refers to Comment x from \revone{Reviewer 1}, and \revtwo{R2.Cx} refers to Comment x from \revtwo{Reviewer 2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\mysectiontitle{Summary of Major Changes}

% \begin{itemize}[leftmargin=0.3cm]
\begin{enumerate}[leftmargin=0.5cm, label=(\Alph*)]

    \item We revised Fig. 1 and Fig. 3, corrected the error in Table II, and added the missing explanation for Step 8 in Fig. 3 (R1.C1, R1.C2, R1.C4). 
    We unified the adversary model terminology to "honest-but-curious" throughout the manuscript (R1.C3). 
    We clarified the mask generation strategy and its resilience to multi-round differential analysis in Section \ref{sec:design} (R1.C5), and addressed the K-means clustering behavior in the absence of malicious clients in Section \ref{sec:design} (R1.C7). 
    We added a discussion on the privacy implications of centered gradients in Section \ref{sec:design} (R1.C6). 
    We added a comparative analysis with HE-based and SMPC-based baselines in Section \ref{sec:complexity_analysis} (R1.C8), and supplemented the privacy analysis with gradient inversion attack experiments in Section \ref{sec:privacy_risk_evaluation} (R1.C9). 

    \item We corrected all typographical errors throughout the manuscript (R2.C2). 
    We conducted scalability experiments and extended the evaluation to the CIFAR-10 dataset with ResNet-18 architecture in Sections \ref{sec:performance} and \ref{sec:robustness_evaluation} (R2.C3, R2.C4). 
    We added a scalability and complexity analysis with HE-based and VSS-based baselines in \ref{fig:scalability} (R2.C5). 
    We clarified the distinction between DP2Guard's non-collusion assumption and that of DPFLA in Section \ref{sec:introduction} (R2.C6), and discussed this limitation in Section VII (R2.C7). We added a sensitivity analysis of $\beta$ in Section \ref{sec:sensitivity_analysis} (R2.C8, R2.C9, R2.C10).

% \end{itemize}
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\mysectiontitle{Response to \revmeta{Associate Editor}}
% \subsection*{Response to \revmeta{Meta-Reviewer}}
\vspace{2mm}

% \begin{myquoteMeta}   
% \rcomment{Associate Editor}{

% }
% \end{myquoteMeta}

\resptometa{AE}{We thank the AE for handling our manuscript. We have carefully revised the paper in response to the reviewers’ comments. Please see the detailed responses below.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\mysectiontitle{Response to \revone{Reviewer \#1}}
\vspace{-2mm}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C1}{
In Fig. 1, it fails to illustrate the claimed property of encrypted gradients being hard to distinguish. The purpose of encryption is to make all gradients computationally indistinguishable from one another, which is precisely what makes it difficult to differentiate benign gradients from malicious ones. However, the existing figure does not convey this fundamental principle—it merely shows that malicious gradients can mislead the global model’s update direction.
}
\end{myquoteR1}
}

\resptoone{R1.C1}{
We thank the reviewer for this concern. We have revised Figure \ref{Fig:PoisoningAttack}.

\begin{modificationR1}{}
    
\end{modificationR1}
\vspace{-10mm}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\linewidth]{figures/fig_1.png}
	\caption{Fig. 1: The example of model poisoning attacks in PPFL. Client 1 uploads a poisoned local mode gradient, guiding the global model towards a predefined direction and impacting overall model performance.}
\end{figure}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C2}{
In Table 1, there appears to be an error in the last row, second column. Based on my reading of the manuscript, the proposed scheme, DP2Guard, does not utilize homomorphic encryption. Please verify and correct this entry.
}
\end{myquoteR1}
}

\resptoone{R1.C2}{
We would like to thank the reviewer for the valuable suggestion. We have revised and corrected the relevant content in Table I.
}

\begin{table}[H]
\caption{TABLE I: Existing Approaches Based on Malicious Client Detection in PPFL}
\label{tb:relatedwork}
\centering
\begin{tabularx}{\textwidth}{|C{2.1cm}|C{2.2cm}|C{2.2cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{2.15cm}|}
\hline
\textbf{Solution} & \textbf{Privacy}& \textbf{Detection approach} & \textbf{Adaptive Aggregation} & \textbf{Test dataset} & \textbf{Blockchain} & \textbf{Byzantine Robustness} & \textbf{Distribution setting} \\
\hline
FLTrust [32] &\Circle & Cosine similarity& \Circle & \Circle & \Circle & \LEFTcircle& IID and Non-IID \\
Multi-Krum [33] &\Circle& Krum & \Circle & \CIRCLE & \Circle & \Circle & IID \\
DnC [31] &\Circle& SVD & \LEFTcircle & \CIRCLE & \Circle & \LEFTcircle & IID \\
RFLP [34] &HE& Krum & \LEFTcircle & \CIRCLE &  \Circle & \LEFTcircle & IID and Non-IID \\
Biscotti [35] &DP& Multi-Krum & \LEFTcircle & \CIRCLE & \CIRCLE & \LEFTcircle & IID \\
% RFLPA \cite{mai2024rflpa} &HE& Cosine similarity & \LEFTcircle & \CIRCLE & \Circle  & \LEFTcircle & IID and Non-IID \\
ShieldFL [37] & Double-trapdoor HE & Cosine similarity & \LEFTcircle & \CIRCLE & \CIRCLE & \LEFTcircle & IID and Non-IID \\
FLOD [26] & SMPC & Hamming distance & \Circle & \Circle & \Circle & \Circle & IID \\
PEFL [7] & HE & Statistical correlation-based & \Circle & \CIRCLE  & \Circle & \Circle & IID \\
VerifyNet [20] & VSS & \Circle & \Circle & \Circle  & \Circle & \Circle & IID \\
DPFLA [38] &Removable mask& SVD & \Circle & \CIRCLE & \Circle & \LEFTcircle & IID \\
\textbf{DP2Guard} &Mask&Hybrid strategy& \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & IID and Non-IID \\
\hline
\end{tabularx}

\vspace{1mm}
\small
\noindent * The symbol \CIRCLE\ indicates YES, \Circle\ indicates NO, \LEFTcircle\ indicates Partially YES. In the column of Byzantine Robustness and Adaptive Aggregation, the half circle \LEFTcircle\ indicates moderate support or defense. A full circle \CIRCLE\ indicates strong support/robustness.

\end{table}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C3}{
 The manuscript uses both "semi-honest" and "curious-but-honest" to describe adversary models. If these terms are intended to describe the same threat model, it is recommended that the terminology be standardized throughout the paper to ensure clarity and consistency of presentation.
}
\end{myquoteR1}
}

\resptoone{R1.C3}{
We thank the reviewer for this suggestion. Here, “semi-honest” and “curious-but-honest” refer to the same threat model, in which clients honestly follow the protocol and submit updates, but may attempt to infer private information from the accessible information. 
To avoid confusion, we have standardized the terminology to "honest-but-curious" throughout the revised manuscript.

% \begin{modificationR1}{}
%     We consider two types of clients: (1) malicious clients; and (2) curious-but-honest clients. Malicious clients deliberately compromise the training process by submitting poisoned gradients aimed at degrading the global model’s accuracy. We assume that the maximum proportion of malicious clients does not exceed half of the total participating devices. In contrast, curious-but-honest clients follow the protocol but may attempt to infer private information from shared local updates, and potentially collaborate with others to improve inference success. 
%     The aggregation process is jointly managed by two servers, S1 and S2, which are assumed to be non-colluding and curious-but-honest—that is, they faithfully execute the protocol but may analyze collected data to recover individual client updates.
%     For the blockchain, we follow a standard Byzantine fault tolerance (BFT) model commonly employed in permissioned blockchain systems [48], [49], where at least $\zeta > 2/3$ of trustee nodes are trustworthy and consistently return correct computation results. For simplicity, we assume all trustees have uniform computational power.
% \end{modificationR1}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C4}{
In Fig. 3, the explanation for Step 8 is missing.
}
\end{myquoteR1}
}

\resptoone{R1.C4}{
We thank the reviewer for pointing this out. The Step 8 label in the original Fig. 3 was a numbering error. We have corrected the step numbering in Fig. 3 in the revised manuscript.
}
\begin{figure}[H]
	\centering
        \includegraphics[width=0.7\linewidth, height=10cm]{figures/fig_3.pdf}
	\captionsetup{labelformat=empty}
    \caption{Fig. 3: A brief workflow of the DP2Guard.}
\end{figure}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C5}{
What is the specific strategy for generating the mask? Could an attacker recover the true gradients through multi-round differential analysis?
}
\end{myquoteR1}
}

\resptoone{R1.C5}{
We thank the reviewer for this comment. 
In \dbname, the mask vector $\mathbf{r}_i$ is independently and uniformly sampled from a continuous random distribution at each communication round by each client. Specifically, each element of $\mathbf{r}_i$ is drawn independently from a uniform distribution over a sufficiently large range. The mask is generated locally on the client device using a pseudo-random number generator (PRNG), and a fresh mask is generated for every round, with no correlation between masks across different rounds or different clients. Regarding the concern about multi-round differential analysis, since each round uses an independently generated mask, the masked gradient shares observed by a server across different rounds are statistically independent. 
Therefore, an attacker cannot accumulate information across rounds to cancel out the masks or infer the true gradients through differential analysis.
Formally, for any two rounds $t_1$ and $t_2$, the mask vectors $\mathbf{r}_i^{\left(t_1\right)}$ and $\mathbf{r}_i^{\left(t_2\right)}$ are independent random variables, and thus $\tilde{\mathbf{g}}_i^{\left(1, t_1\right)}-\tilde{\mathbf{g}}_i^{\left(1, t_2\right)}=\left(\mathbf{g}_i^{\left(t_1\right)}-\mathbf{g}_i^{\left(t_2\right)}\right)+\left(\mathbf{r}_i^{\left(t_1\right)}-\mathbf{r}_i^{\left(t_2\right)}\right)$, where the difference of two independent random masks remains a random variable that conceals the true gradient difference.

We have clarified the mask generation strategy and added a discussion of its resilience to multi-round differential analysis in Section \ref{sec:design} of the revised manuscript.

\begin{modificationR1}
\textbf{2) Local Model Training:} In the $t$-th communication round, each edge device $E_i$ updates its local model by training on its private dataset using the global model parameters $\mathbf{w}^{(t-1)}$ retrieved from the blockchain. After completing local training, the device computes its local gradient update $\mathbf{g}_i^{(t)}$. To protect the privacy of this gradient, DP2Guard designs a gradient splitting and masking strategy. Specifically, edge device $E_i$ first splits its gradient $\mathbf{g}_i$ into two additive shares $\mathbf{g}_i^{(1)}$ and $\mathbf{g}_i^{(2)}$, such that $\mathbf{g}_i=\mathbf{g}_i^{(1)}+\mathbf{g}_i^{(2)}$. 
To obfuscate the true gradient values, each device independently generates a fresh random mask vector $\mathbf{r}_i \in \mathbb{R}^{m \times n}$ at each communication round using a pseudo-random number generator (PRNG), where each element is independently and uniformly sampled. 
The mask generation is performed entirely locally on the device, without requiring any key agreement or coordination with other clients or servers.
Using this mask vector, the device creates two masked gradient shares:
\begin{equation}
    \tilde{\mathbf{g}}_i^{(1)}=\mathbf{g}_i^{(1)}+\mathbf{r}_i, \quad \tilde{\mathbf{g}}_i^{(2)}=\mathbf{g}_i^{(2)}-\mathbf{r}_i.
\end{equation}


These masked gradients are transmitted separately to Servers S1 and S2. This mechanism effectively safeguards against direct gradient leakage, no single server can infer the original gradient or any intermediate component without collaboration. The detailed procedure for this gradient splitting and masking process is presented in Algorithm 1.

\textit{Remark.}
Since each client generates its mask vector independently and locally, no inter client communication or key negotiation is required, resulting in $O(N)$ communication complexity, which is significantly more efficient than secure aggregation protocols (e.g., SecAgg [42]) that require pairwise key agreement with $O\left(N^2\right)$ overhead. 
Furthermore, a fresh mask vector is independently generated at each round, ensuring statistical independence across rounds and preventing attackers from recovering true gradients through multi-round differential analysis. 
Specifically, for any two rounds $t_1$ and $t_2$, the difference $\tilde{\mathbf{g}}_i^{\left(1, t_1\right)}-\tilde{\mathbf{g}}_i^{\left(1, t_2\right)}=\left(\mathbf{g}_i^{\left(t_1\right)}-\mathbf{g}_i^{\left(t_2\right)}\right)+\left(\mathbf{r}_i^{\left(t_1\right)}-\mathbf{r}_i^{\left(t_2\right)}\right)$ remains masked by the difference of two independent random vectors, which cannot be eliminated.
\end{modificationR1}

}



\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C6}{
Can the centered gradients reconstructed by server $S_2$ reveal or allow inference of any sensitive information?
}
\end{myquoteR1}
}

\resptoone{R1.C6}{
We thank the reviewer for this comment. In \dbname,  server $S_2$ observes the centered gradients $\hat{\mathbf{g}}_i=\mathbf{g}_i-\overline{\mathbf{g}}$ for each client during the detection phase, which represents the deviation from the global mean rather than the raw gradient $\mathbf{g}_i$ itself. 
Since $S_2$ does not have access to the global mean $\overline{\mathbf{g}}$, the absolute value of $\mathbf{g}_i$ remains hidden. 
Recovering $\mathbf{g}_i$ would require knowledge of $\overline{\mathbf{g}}$, which in turn would necessitate colluding with $S_1$ or accessing all clients' original gradients, both of which are precluded by our threat model.
Therefore, the mean-centering approach ensures that $S_2$ only obtains the relative differences among client gradients, without revealing any individual client's raw gradient. 

We have added a detailed discussion in Section \ref{sec:design} of the revised manuscript. 
Furthermore, to provide empirical evidence, we have conducted gradient inversion attack experiments using the DLG algorithm, with results presented in Section \ref{sec:privacy_risk_evaluation}. The results confirm that the centered gradients are insufficient for successful gradient reconstruction.
\begin{modificationR1}{}

To evaluate the privacy-preserving effectiveness of DP2Guard, we conduct gradient inversion attacks using the DLG (Deep Leakage from Gradients) [59] algorithm, which attempts to reconstruct private training data from observed gradients. Experiments are performed on both the MNIST and CIFAR-10 datasets.

We first compare DP2Guard with ShieldFL and FedAvg under the standard honest-but-curious server model. As shown in Fig. \ref{fig:gradient_inversion}, FedAvg, which provides no privacy protection, allows the attacker to successfully reconstruct recognizable training images. 
In contrast, both ShieldFL and DP2Guard effectively prevent gradient reconstruction, with the reconstructed images being indistinguishable from random noise. These results demonstrate that the lightweight gradient splitting and masking mechanism in DP2Guard provides privacy protection comparable to the HE-based approach adopted by ShieldFL.

We further evaluate the privacy resilience under a more challenging server-client collusion scenario, comparing DP2Guard with DPFLA. As shown in Fig. \ref{fig:gradient_inversion_collusion}, when a server colludes with a client, DPFLA fails to protect gradient privacy, and the attacker can successfully reconstruct recognizable training images. 
Under the same collusion setting, DP2Guard exhibits some residual visual features in the reconstructed images; however, the reconstruction quality is severely degraded and insufficient for a successful attack. 
This is because DP2Guard only requires non-collusion between the two servers $S_1$ and $S_2$, and does not rely on the assumption of non-collusion between servers and clients. 
These results confirm that DP2Guard provides stronger privacy protection than DPFLA even under server-client collusion.

\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/comparison_mnist.eps}
        \caption{MNIST dataset.}
        \label{fig:gradinv_noenc}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/comparison_cifar10.eps}
        \caption{CIFAR-10 dataset.}
        \label{fig:gradinv_paillier}
    \end{subfigure}
    \captionsetup{labelformat=empty}
    \caption{Fig. 6: Visual comparison of images reconstructed by the DLG attack under different defense mechanisms on MNIST and CIFAR-10 datasets.}
    \label{fig:gradient_inversion}
\end{figure}
\vspace{-8mm}
\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/collusion_mnist.eps}
        \caption{MNIST dataset.}
        \label{fig:gradinv_noenc}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/collusion_cifar10.eps}
        \caption{CIFAR-10 dataset.}
        \label{fig:gradinv_paillier}
    \end{subfigure}
    \captionsetup{labelformat=empty}
    \caption{Fig. 7: Visual comparison of images reconstructed by the DLG attack under server-client collusion between DPFLA and DP2Guard on MNIST and CIFAR-10 datasets.}
    \label{fig:gradient_inversion_collusion}
\end{figure}
\end{modificationR1}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C7}{
Using K-means clustering (with K=2) to differentiate between malicious and benign gradients is an intuitive approach. However, it presents a potential flaw: in training rounds where no malicious gradients are present, the algorithm would still forcibly partition the gradients into two clusters, thereby creating a "false malicious" class. How does the proposed scheme address this issue?
}
\end{myquoteR1}
}

\resptoone{R1.C7}{
We thank the reviewer for this comment. 
In our implementation, a cluster separation check is performed after K-means clustering to handle the case where no malicious clients are present. 
Specifically, we compute the Euclidean distance between the two cluster centroids $D=\|\mu_1-\mu_2\|$ and compare it with an adaptive threshold $\epsilon$, which is determined based on the intra-cluster distances in each round: $\epsilon=\alpha \cdot \frac{1}{2}\left(\bar{d}_1+\bar{d}_2\right)$, where $\bar{d}_1$ and $\bar{d}_2$ are the average distances from data points to their respective centroids, and $\alpha$ is a scaling factor set to 2 in our experiments. 
If $D<\epsilon$, the two clusters are considered insufficiently separated, and all clients are treated as benign in that round. 
Only when $D \geq \epsilon$ are clients in the smaller cluster excluded as potentially malicious. 
By using an adaptive threshold rather than a fixed value, the separation check automatically adjusts to different data distributions across datasets and training rounds.

We have clarified this detail in Section \ref{sec:design} of the revised manuscript. 

\begin{modificationR1}
\textbf{Clustering-Based Detection:} Next, a two-dimensional feature vector is constructed for each client:
\begin{equation}
    \mathbf{f}_i=\left[s_i, c_i\right]^{\top}
\end{equation}
A K-means clustering algorithm [51] with $K=2$ is applied to these features, producing two clusters $\mathcal{C}_1$ and $\mathcal{C}_2$ with centroids $\boldsymbol{\mu}_1$ and $\boldsymbol{\mu}_2$, respectively. To ensure reliable detection, a cluster separation check is performed. We compute the Euclidean distance between the two centroids:
$$
D=\left\|\mu_1-\mu_2\right\|
$$
and compare it with an adaptive threshold $\epsilon$ derived from the intra-cluster distances:
$$
\epsilon=\alpha \cdot \frac{1}{2}\left(\bar{d}_1+\bar{d}_2\right)
$$
where $\bar{d}_1=\frac{1}{\left|\mathcal{C}_1\right|} \sum_{\mathbf{f}_j \in \mathcal{C}_1}\left\|\mathbf{f}_j-\boldsymbol{\mu}_1\right\|$ and $\bar{d}_2=\frac{1}{\left|\mathcal{C}_2\right|} \sum_{\mathbf{f}_j \in \mathcal{C}_2}\left\|\mathbf{f}_j-\boldsymbol{\mu}_2\right\|$ denote the average intra-cluster distances, and $\alpha>1$ is a scaling factor. If $D<\epsilon$, the inter-cluster separation is smaller than the intra-cluster spread, indicating that all clients exhibit similar behavior in the current round. In this case, all clients are treated as benign and included in aggregation. If $D \geq \epsilon$, clients in the larger cluster are considered benign, while those in the smaller cluster are identified as anomalous and excluded from aggregation. This adaptive separation check avoids false exclusion of benign clients in attack-free rounds while maintaining effective detection when attacks are present.

\end{modificationR1}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C8}{
The manuscript emphasizes that the proposed scheme is lightweight, but this claim lacks sufficient justification. Although a complexity analysis of the proposed scheme's operations is provided, it lacks a comparative analysis against other established solutions (e.g., those based on Homomorphic Encryption or Multi-Party Computation). To strengthen this claim, I suggest adding both qualitative and quantitative comparisons with relevant baselines to provide readers with a clearer understanding of the proposed scheme's efficiency.
}
\end{myquoteR1}
}

\resptoone{R1.C8}{
We thank the reviewer for this comment. Following your suggestion, we have added a efficiency comparison with established privacy-preserving FL baselines in Section \ref{sec:complexity_analysis} of the revised manuscript. Specifically, we compare DP2Guard with HE-based schemes (PEFL [38] and ShieldFL [37]) and a SMPC-based scheme (VerifyNet [20]). For the qualitative comparison, Table VI presents the theoretical computational and communication complexity of all schemes on both the server and client sides. The analysis shows that DP2Guard achieves the lowest client-side computation at $\mathcal{O}(d T_{\text {prg}})+\mathcal{O}(d T_{\text {add}})$, compared to $\mathcal{O}(d T_{\text {phe}})$ for HE-based schemes and $\mathcal{O}(d N T_{\text {vss}})$ for VerifyNet. 
For the quantitative comparison, Fig. 8 reports the per-round computation time and communication cost breakdown, and Fig. 9 evaluates the scalability under different numbers of clients. 
The results demonstrate that DP2Guard introduces minimal overhead beyond FedAvg, while ShieldFL, PEFL, and VerifyNet incur substantially higher computation and communication costs due to ciphertext operations and inter-client interactions. 
These comparisons provide concrete evidence supporting the lightweight advantage of DP2Guard.

\begin{modificationR1}{}
We evaluate the efficiency of DP2Guard from both theoretical complexity and runtime overhead perspectives.

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\captionsetup{labelformat=empty}
\caption{TABLE II: Comparison of computational and communication complexity.}
\label{tab:cost_analysis}
\begin{tabular}{lccccc}
\toprule
\textbf{Scheme} & \textbf{Technique} & \multicolumn{2}{c}{\textbf{Computation}} & \multicolumn{2}{c}{\textbf{Communication}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 & & \textbf{Server} & \textbf{Client} & \textbf{Server} & \textbf{Client} \\
\midrule
PEFL 
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
VerifyNet
& VSS
& $\mathcal{O}(n^2 d T_{\text{vss}})$
& $\mathcal{O}(dN T_{\text{vss}})$
& $\mathcal{O}((n^2+nd)|\omega_{\text{vss}}|)$
& $\mathcal{O}((N+d)|\omega_{\text{vss}}|)$ \\
ShieldFL 
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
DP2Guard
& GSM
& $\mathcal{O}(n^2 d T_{\text{add}})$
& $\mathcal{O}(d T_{\text{prg}}) + \mathcal{O}(d T_{\text{add}})$
& $\mathcal{O}(nd|\omega|)$
& $\mathcal{O}(2d|\omega|)$ \\
\bottomrule
\end{tabular}
\vspace{2pt}
\begin{tablenotes}
\footnotesize
\item PHE: partially homomorphic encryption; GSM: gradient splitting and masking; VSS: verifiable secret sharing. $d$: gradient dimension; $n$: number of clients. $T_{\text{prg}}$: cost of generating a pseudo-random number; $T_{\text{add}}$: cost of a plaintext addition; $T_{\text{phe}}$: cost of a PHE encryption ($T_{\text{phe}} \gg T_{\text{add}}$); $T_{\text{vss}}$: cost of generating a VSS share. $|\omega|$: size of a plaintext number; $|\omega_{\text{phe}}|$: size of a PHE ciphertext ($|\omega_{\text{phe}}| \gg |\omega|$); $|\omega_{\text{vss}}|$: size of a VSS share.
\end{tablenotes}
\end{table}

\textbf{Complexity Analysis:} Table \ref{tab:cost_analysis} summarizes the computational and communication complexity of DP2Guard compared with state-of-the-art schemes: PEFL [37], VerifyNet [20], and ShieldFL [38]. 
On the client side, DP2Guard requires $\mathcal{O}(d T_{\text {prg}})+\mathcal{O}(d T_{\text {add }})$ computation for pseudo-random mask generation and gradient splitting, where $T_{\text {prg }}$ denotes the cost of generating a pseudo-random number and $T_{\text {add }}$ denotes the cost of a single addition operation.
These are lightweight arithmetic operations without any cryptographic overhead. 
In contrast, PEFL and ShieldFL require $\mathcal{O}(d T_{\text {phe}})$ due to per-element PHE encryption, where $T_{\text {phe}} \gg T_{\text {add}}$, and VerifyNet incurs $\mathcal{O}(d N T_{\text {vss}})$ due to per-element verifiable secret sharing across $N$ clients. 
For communication, DP2Guard transmits two plaintext masked gradient shares at $\mathcal{O}(2d|\omega|)$, where $|\omega|$ is the size of a single plaintext number. 
PEFL and ShieldFL transmit HE ciphertexts at $\mathcal{O}(d|\omega_{\text {phe}}|)$, where $|\omega_{\text{phe }}| \gg|\omega|$ due to ciphertext expansion. VerifyNet requires $\mathcal{O}((N+d N)|\omega_{\text {vss }}|)$ due to inter-client secret sharing. 
On the server side, the computation of DP2Guard is dominated by pairwise cosine similarity at $\mathcal{O}(n^2d T_{\text {add }})$, performed entirely in plaintext. 
ShieldFL and PEFL perform analogous pairwise operations on HE ciphertexts at $\mathcal{O}(n^2 d T_{\text {phe }})$, resulting in substantially higher actual computation time since $T_{\text {phe }}$ is orders of magnitude larger than $T_{\text {add}}$.


\textbf{Runtime Overhead:} To further validate the efficiency advantage of DP2Guard, we measure the actual computation time and communication cost per training round, comparing DP2Guard with PEFL, VerifyNet, and ShieldFL. 

Fig. \ref{fig:breakdown_comp} presents the per-round execution time breakdown across different phases: local model training, gradient privacy protection, poisoning detection, and secure aggregation. The results show that ShieldFL incurs the highest overhead, followed by PEFL, both due to HE ciphertext operations in the secure aggregation phase. VerifyNet introduces significant overhead in the gradient privacy protection phase due to inter-client secret sharing and verification. In contrast, DP2Guard introduces minimal overhead beyond FedAvg, as its gradient splitting and masking operations require only lightweight plaintext arithmetic without any cryptographic operations.
Fig. \ref{fig:breakdown_comm} shows the communication overhead comparison. DP2Guard transmits plaintext masked gradient shares, resulting in substantially lower communication cost compared to VerifyNet and ShieldFL, which are dominated by inter-client secret sharing messages and HE ciphertexts, respectively. PEFL incurs moderate communication overhead due to ciphertext transmission.

\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/overhead_computation.png}
    \caption{Computation Cost}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/overhead_communication.png}
    \caption{Communication Cost}
\end{subfigure}
\captionsetup{labelformat=empty}
\caption{Fig. 8: Per-iteration overhead comparison under 40\% Byzantine clients.}
\label{fig:breakdown}
\end{figure}
\vspace{-8mm}
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/scalability_computation.png}
    \caption{Computation Cost}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/scalability_communication.png}
    \caption{Communication Cost}
\end{subfigure}
\captionsetup{labelformat=empty}
\caption{Fig. 9: Computational and communication overheads for different numbers of clients.}
\label{fig:scalability}
\end{figure}
\end{modificationR1}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR1}
\rcomment{R1.C9}{
To provide a more direct and empirical demonstration of the proposed scheme's privacy-preserving capabilities, I suggest supplementing the analysis with the results of simulated privacy attacks. Evaluating the extent of privacy leakage when the system is exposed to attacks launched by a curious-but-honest server—such as membership inference, property inference, and model inversion—would significantly strengthen the paper's claims.
}
\end{myquoteR1}
}

\resptoone{R1.C9}{
We thank the reviewer for this comment. To provide empirical evidence of DP2Guard's privacy-preserving capabilities, we have conducted gradient inversion attack experiments in the revised manuscript. Specifically, we adopt the DLG [59] algorithm as a representative model inversion attack, where an honest-but-curious server attempts to reconstruct clients' private training data from the gradients it can observe. 
 Experiments are performed on both MNIST and CIFAR-10 datasets. We first compare DP2Guard with ShieldFL and FedAvg under the standard honest-but-curious server model. 
 As shown in Fig. 6, FedAvg allows the attacker to successfully reconstruct recognizable training images, while both ShieldFL and DP2Guard effectively prevent reconstruction, with the results indistinguishable from random noise. 
 We further evaluate the privacy resilience under a server-client collusion scenario, comparing DP2Guard with DPFLA. As shown in Fig. 7, DPFLA fails to protect gradient privacy under collusion, whereas DP2Guard maintains substantially degraded reconstruction quality insufficient for a successful attack. 
 
 These results are presented in Section \ref{sec:privacy_risk_evaluation} of the revised manuscript.

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\vspace{-3mm}
\mysectiontitle{Response to \revtwo{Reviewer \#2}}
\vspace{-2mm}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C1}{
- This paper proposes DP2Guard to achieve four objectives: maintaining high test accuracy without degradation by privacy preservation, minimizing communication/computation costs, ensuring robustness against poisoning attacks, and preserving privacy against inference attacks.

- The authors present gradient splitting and masking, hybrid defense, and trust-weighted adaptive aggregation.

- The authors evaluate DP2Guard on publicly known datasets and model architectures against four poisoning attack types.

[Strengths]
- DP2Guard's objectives and evaluation metrics are straightforward and practical.

- The paper (Especially Section II) is well-organized.

- The paper includes enough background, making it easy to read.
}
\end{myquoteR2}
}

\resptotwo{R2.C1}{
We appreciate the reviewer' positive evaluation of our work. Following the reviewer’s subsequent suggestions, we have further improved the revised manuscript.
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C2}{
There are too many typos: pg.1 'similarity-based similarity-based' (Duplicated); Fig. 1 'Begin' (Should be 'Benign'); pg. 4 'random vector $m_i$' (Should be $r_i$); Table 2 'i clients' (Should be 'Client i'); Table 2 'Mean-centering gradient' (Should be 'Mean-centered gradient'); pg.5 'DP2Guard troduces' (Should be 'introduces'); Fig. 3 'Begin' (Should be 'Benign'); Fig. 3 $\lambda$ (Should be $\tau$); pg. 8 DP2Gurd (Should be 'DP2Guard').
}
\end{myquoteR2}
}

\resptotwo{R2.C2}{
We thank the reviewer for this comment. We have addressed the issues noted above and thoroughly reviewed the entire manuscript to ensure consistency in the text and figures.
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C3}{
The 50 clients used in the experiments do not appear to be a particularly large number. Since the paper mentions communication overhead as a drawback of SMPC when the number of clients increases, it would be important to either (i) demonstrate that SMPC already incurs significant communication overhead even with 50 clients, or (ii) show that DP2Guard maintains strong performance even with a substantially larger number of clients.
}
\end{myquoteR2}
}

\resptotwo{R2.C3}{
We thank the reviewer for this suggestion. We address this concern from both perspectives. First, we have added a comprehensive efficiency comparison with HEbased schemes (PEFL and ShieldFL) and a VSS-based scheme (VerifyNet) in Section \ref{sec:complexity_analysis}. 
The per-round overhead breakdown in Fig. 8 demonstrates that even with a moderate number of clients, these schemes already incur substantial computation and communication overhead compared to DP2Guard. For instance, ShieldFL requires significantly more computation time per round than DP2Guard, with the gap primarily driven by ciphertextdomain operations. Second, we have conducted scalability experiments with $N \in$ \{50,100,150,200\} clients on both MNIST and CIFAR-10 datasets. As shown in Fig. 9, both the computation time and communication cost of DP2Guard grow linearly with the number of clients, remaining close to FedAvg across all scales. In contrast, VerifyNet exhibits nearquadratic growth, and ShieldFL and PEFL incur substantially higher overhead at all scales due to HE ciphertext operations. These results confirm that DP2Guard maintains strong efficiency even as the number of clients increases, while HE-based and VSS-based approaches become increasingly impractical at larger scales.

\begin{modificationR2}{}
We evaluate the efficiency of DP2Guard from both theoretical complexity and runtime overhead perspectives.

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\captionsetup{labelformat=empty}
\caption{TABLE V: Comparison of computational and communication complexity.}
\label{tab:cost_analysis}
\begin{tabular}{lccccc}
\toprule
\textbf{Scheme} & \textbf{Technique} & \multicolumn{2}{c}{\textbf{Computation}} & \multicolumn{2}{c}{\textbf{Communication}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 & & \textbf{Server} & \textbf{Client} & \textbf{Server} & \textbf{Client} \\
\midrule
PEFL
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
VerifyNet 
& VSS
& $\mathcal{O}(n^2 d T_{\text{vss}})$
& $\mathcal{O}(dN T_{\text{vss}})$
& $\mathcal{O}((n^2+nd)|\omega_{\text{vss}}|)$
& $\mathcal{O}((N+d)|\omega_{\text{vss}}|)$ \\
ShieldFL
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
DP2Guard
& GSM
& $\mathcal{O}(n^2 d T_{\text{add}})$
& $\mathcal{O}(d T_{\text{prg}}) + \mathcal{O}(d T_{\text{add}})$
& $\mathcal{O}(nd|\omega|)$
& $\mathcal{O}(2d|\omega|)$ \\
\bottomrule
\end{tabular}
\vspace{2pt}
\begin{tablenotes}
\footnotesize
\item PHE: partially homomorphic encryption; GSM: gradient splitting and masking; VSS: verifiable secret sharing. $d$: gradient dimension; $n$: number of clients. $T_{\text{prg}}$: cost of generating a pseudo-random number; $T_{\text{add}}$: cost of a plaintext addition; $T_{\text{phe}}$: cost of a PHE encryption ($T_{\text{phe}} \gg T_{\text{add}}$); $T_{\text{vss}}$: cost of generating a VSS share. $|\omega|$: size of a plaintext number; $|\omega_{\text{phe}}|$: size of a PHE ciphertext ($|\omega_{\text{phe}}| \gg |\omega|$); $|\omega_{\text{vss}}|$: size of a VSS share.
\end{tablenotes}
\end{table}

\textbf{Complexity Analysis:} Table \ref{tab:cost_analysis} summarizes the computational and communication complexity of DP2Guard compared with state-of-the-art schemes: PEFL [37], VerifyNet [20], and ShieldFL [38]. 
On the client side, DP2Guard requires $\mathcal{O}(d T_{\text {prg}})+\mathcal{O}(d T_{\text {add }})$ computation for pseudo-random mask generation and gradient splitting, where $T_{\text {prg }}$ denotes the cost of generating a pseudo-random number and $T_{\text {add }}$ denotes the cost of a single addition operation.
These are lightweight arithmetic operations without any cryptographic overhead. 
In contrast, PEFL and ShieldFL require $\mathcal{O}(d T_{\text {phe}})$ due to per-element PHE encryption, where $T_{\text {phe}} \gg T_{\text {add}}$, and VerifyNet incurs $\mathcal{O}(d N T_{\text {vss}})$ due to per-element verifiable secret sharing across $N$ clients. 
For communication, DP2Guard transmits two plaintext masked gradient shares at $\mathcal{O}(2d|\omega|)$, where $|\omega|$ is the size of a single plaintext number. 
PEFL and ShieldFL transmit HE ciphertexts at $\mathcal{O}(d|\omega_{\text {phe}}|)$, where $|\omega_{\text{phe }}| \gg|\omega|$ due to ciphertext expansion. VerifyNet requires $\mathcal{O}((N+d N)|\omega_{\text {vss }}|)$ due to inter-client secret sharing. 
On the server side, the computation of DP2Guard is dominated by pairwise cosine similarity at $\mathcal{O}(n^2d T_{\text {add }})$, performed entirely in plaintext. 
ShieldFL and PEFL perform analogous pairwise operations on HE ciphertexts at $\mathcal{O}(n^2 d T_{\text {phe }})$, resulting in substantially higher actual computation time since $T_{\text {phe }}$ is orders of magnitude larger than $T_{\text {add}}$.

\textbf{Runtime Overhead:} To further validate the efficiency advantage of DP2Guard, we measure the actual computation time and communication cost per training round, comparing DP2Guard with PEFL, VerifyNet, and ShieldFL. 


Fig. \ref{fig:breakdown_comp} presents the per-round execution time breakdown across different phases: local model training, gradient privacy protection, poisoning detection, and secure aggregation. The results show that ShieldFL incurs the highest overhead, followed by PEFL, both due to HE ciphertext operations in the secure aggregation phase. VerifyNet introduces significant overhead in the gradient privacy protection phase due to inter-client secret sharing and verification. In contrast, DP2Guard introduces minimal overhead beyond FedAvg, as its gradient splitting and masking operations require only lightweight plaintext arithmetic without any cryptographic operations.
Fig. \ref{fig:breakdown_comm} shows the communication overhead comparison. DP2Guard transmits plaintext masked gradient shares, resulting in substantially lower communication cost compared to VerifyNet and ShieldFL, which are dominated by inter-client secret sharing messages and HE ciphertexts, respectively. PEFL incurs moderate communication overhead due to ciphertext transmission.


\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/overhead_computation.png}
    \caption{Computation Cost}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/overhead_communication.png}
    \caption{Communication Cost}
\end{subfigure}
\captionsetup{labelformat=empty}
\caption{Fig. 8: Per-iteration overhead comparison under 40\% Byzantine clients.}
\label{fig:breakdown}
\end{figure}
\vspace{-8mm}
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/scalability_computation.png}
    \caption{Computation Cost}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{result/overhead/scalability_communication.png}
    \caption{Communication Cost}
\end{subfigure}
\captionsetup{labelformat=empty}
\caption{Fig. 9: Computational and communication overheads for different numbers of clients.}
\label{fig:scalability}
\end{figure}

\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C4}{
The experiments are limited to small-scale datasets and model architectures, leaving uncertainty as to whether DP2Guard can also benefit in larger-scale or more complex real-world scenarios.
}
\end{myquoteR2}
}

\resptotwo{R2.C4}{
We thank the reviewer for this suggestion. Following your suggestion, we have extended our experimental evaluation on the CIFAR-10 dataset, which contains 60,000 color images of size $32 \times 32$ across 10 classes and presents substantially greater complexity than the grayscale datasets used previously. Correspondingly, we have adopted the ResNet-18 model architecture, which is significantly deeper and more representative of practical deep learning applications compared to LeNet-5.  
The results, presented in Table III, Table IV, and Fig. 4, demonstrate that DP2Guard maintains strong defense performance and model accuracy on the more complex dataset and model architecture across all attack types under both IID and Non-IID settings, confirming its effectiveness beyond small-scale settings. 

We have updated the experimental evaluation in Sections \ref{sec:performance} and \ref{sec:robustness_evaluation} of the revised manuscript.

\begin{modificationR2}
\textbf{Datasets and Model Architectures:} We evaluate our proposed scheme on three benchmark datasets: MNIST, Fashion-MNIST, and CIFAR-10. 
The MNIST dataset contains 60,000 training and 10,000 testing grayscale images of handwritten digits, each of size $28 \times 28$ pixels and classified into 10 categories. 
The Fashion-MNIST dataset consists of 60,000 training and 10,000 testing grayscale images representing various types of clothing items, also distributed across 10 classes. 
The CIFAR-10 dataset contains 50,000 training and 10,000 testing color images of size $32 \times 32$ pixels across 10 classes. 
For MNIST and Fashion-MNIST, we employ the LeNet5 model [54] to perform the training tasks.
For CIFAR-10, we adopt the deeper ResNet18 model [55] to better handle the increased complexity of the color image dataset. For all experiments,
we adopt stochastic gradient descent (SGD) as the optimizer, with a learning rate $\eta=0.01$ and a batch size of 32.

\textit{1) Accuracy evaluation:} To evaluate the convergence efficiency of different aggregation algorithms, we conducted experiments over 300 global communication rounds on the MNIST, Fashion-MNIST, and CIFAR-10 datasets under a no-attack scenario, using both IID and non-IID data settings. As shown in Fig. \ref{fig:performance}, all methods achieve high final accuracy under the IID setting on MNIST and Fashion-MNIST. However, DP2Guard stabilizes within the first 50 rounds, whereas FedAvg and MultiKrum typically require over 100 rounds to converge. 
Under the non-IID setting, the performance gap widens. In particular, on the Fashion-MNIST dataset, FedAvg and MultiKrum show noticeable fluctuations during training, indicating sensitivity to data heterogeneity. 
In contrast, ShieldFL and DP2Guard exhibit smoother convergence curves. 
On the CIFAR-10 dataset with ResNet-18, all methods exhibit slower convergence due to the increased model complexity and data diversity. 
Nevertheless, DP2Guard consistently achieves competitive final accuracy and demonstrates more stable convergence compared to other baselines under both IID and non-IID settings. 

\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/mnist_lenet_iid_noattack_ieee.png}
\caption{MNIST (IID)}
\label{fig:perf_a}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/mnist_lenet_non_iid_noattack_ieee.png}
\caption{MNIST (Non-IID)}
\label{fig:perf_b}
\end{subfigure}
\captionsetup{labelformat=empty}
% \caption{Fig. 9: Computational and communication overheads for different numbers of clients.}
\label{fig:scalability}
\end{figure}
\vspace{-15mm}
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/fashion_lenet_iid_noattack_ieee.png}
\caption{Fashion-MNIST (IID)}
\label{fig:perf_c}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/fashion_lenet_non_iid_noattack_ieee.png}
\caption{Fashion-MNIST (Non-IID)}
\label{fig:perf_d}
\end{subfigure}
\captionsetup{labelformat=empty}
% \caption{Fig. 9: Computational and communication overheads for different numbers of clients.}
\label{fig:scalability}
\end{figure}
\vspace{-15mm}
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/cifar_resnet_iid_noattack_ieee.png}
\caption{CIFAR10 (IID)}
\label{fig:perf_c}
\end{subfigure}
\hspace{3mm}
\begin{subfigure}[t]{0.33\columnwidth}
\centering
\includegraphics[width=\linewidth]{result/cifar_resnet_non_iid_noattack_ieee.png}
\caption{CIFAR10 (Non-IID)}
\label{fig:perf_d}
\end{subfigure}
\caption{Fig. 4: Impact of training iterations on the effectiveness of defense strategies on MNIST and Fashion-MNIST datasets under IID and Non-IID settings.}
\end{figure}


% \begin{figure}[H]
% \centering
% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/mnist_lenet_iid_noattack_ieee.png}
% \caption{MNIST (IID)}
% \label{fig:perf_a}
% \end{subfigure}
% \hspace{3mm}
% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/mnist_lenet_non_iid_noattack_ieee.png}
% \caption{MNIST (Non-IID)}
% \label{fig:perf_b}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/fashion_lenet_iid_noattack_ieee.png}
% \caption{Fashion-MNIST (IID)}
% \label{fig:perf_c}
% \end{subfigure}
% \hspace{3mm}
% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/fashion_lenet_non_iid_noattack_ieee.png}
% \caption{Fashion-MNIST (Non-IID)}
% \label{fig:perf_d}
% \end{subfigure}

% \vspace{2mm}

% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/cifar_resnet_iid_noattack_ieee.png}
% \caption{CIFAR10 (IID)}
% \label{fig:perf_c}
% \end{subfigure}
% \hspace{3mm}
% \begin{subfigure}[t]{0.35\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{result/cifar_resnet_non_iid_noattack_ieee.png}
% \caption{CIFAR10 (Non-IID)}
% \label{fig:perf_d}
% \end{subfigure}

% \caption{Fig. 4: Impact of training iterations on the effectiveness of defense strategies on MNIST and Fashion-MNIST datasets under IID and Non-IID settings.}
% \label{fig:performance}
% \end{figure}

\textit{2) Robustness:} To comprehensively evaluate the robustness of DP2Guard, we compare all defense methods against four representative poisoning attacks: Label Flipping (LF), Fang, Min-Max, and Min-Sum, with malicious-client ratios ranging from 10\% to 40\%. 
Experiments are conducted on MNIST, Fashion-MNIST, and CIFAR-10 datasets under both IID and Non-IID settings. The results are summarized in Table \ref{tab:def_per_iid} and Table \ref{tab:def_per_noniid}.

\textbf{Performance under IID setting.} As shown in Table \ref{tab:def_per_iid}, DP2Guard consistently achieves the highest accuracy across all datasets, attack types, and malicious-client ratios. On the MNIST dataset, DP2Guard maintains accuracy above 95\% even under 40\% adversary ratio across all four attacks, while FedAvg drops sharply under Fang attack (from 90.0\% to 10.1\%) and MultiKrum degrades significantly under Min-Max and Min-Sum attacks. On Fashion-MNIST, the performance gap becomes more evident. Under the Fang attack with 40\% adversaries, FedAvg collapses to 10.0\% and MultiKrum falls to 47.2\%, whereas DP2Guard retains 78.2\%, outperforming ShieldFL (74.2\%) and DnC (73.9\%). On the more complex CIFAR-10 dataset, all methods exhibit lower overall accuracy due to the increased task difficulty. Nevertheless, DP2Guard consistently leads, achieving 72.4\% under LF attack, 71.0\% under Fang attack, 72.2\% under Min-Max attack, and 72.7\% under Min-Sum attack at 40\% adversary ratio, surpassing all baselines by 1\%--4\%. Notably, DP2Guard demonstrates the smallest accuracy degradation as the poisoning ratio increases, indicating strong resilience against escalating adversarial threats.
\newcommand{\best}[1]{\cellcolor{gray!25}\textbf{#1}}
\newcommand{\sbest}[1]{\cellcolor{gray!10}{#1}}

\begin{table}[H]
\centering
\caption{TABLE III: Comparison of defense strategies against four poisoning attacks on MNIST, Fashion-MNIST, and CIFAR-10 in the IID setting, with malicious-client ratios ranging from 10\% to 40\%.}
\label{tab:def_per_iid}
\resizebox{\textwidth}{!}{%
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.35}
\begin{tabular}{ll cccc cccc cccc cccc}
\toprule
\multirow{2}{*}{\textbf{Data set}} & \multirow{2}{*}{\textbf{Method}}
& \multicolumn{4}{c}{\textbf{LF Attack}}
& \multicolumn{4}{c}{\textbf{Fang Attack}}
& \multicolumn{4}{c}{\textbf{Min-Max}}
& \multicolumn{4}{c}{\textbf{Min-Sum Attack}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}

&
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}\\
\midrule

\multirow{6}{*}{\textbf{MNIST}}
    & FedAvg     & 95.2 & 93.4 & 90.1 & 85.3  & 90.0 & 84.2 & 65.4 & 10.1 & 95.0 & 92.4 & 87.0 & 80.3  & 94.0 & 90.4 & 86.0 & 82.9 \\
    & FLTrust    & 96.5 & 96.2 & 95.9 & 94.6 & \best{96.4} & \sbest{95.0} & 94.0 & \sbest{93.4}  & 95.9 & 95.2 & 94.7 & 94.1  & 96.0 & 95.4 & 95.0 & 94.7 \\
    & MultiKrum  & 96.0 & 95.8 & 95.4 & 94.0  & 95.1 & 90.8 & 85.2 & 74.3  & 96.2 & 95.0 & 94.0 & 85.5  & 95.7 & 94.0 & 92.0 & 86.3 \\
    & ShieldFL  & 96.9 & \sbest{96.6} & 96.24 & 94.5 & \sbest{96.0} & \best{95.4} & \sbest{94.1} & \sbest{93.3} & \sbest{96.8} & \sbest{96.0} & \sbest{95.2} & \sbest{94.4} & \sbest{96.5} & \sbest{96.0} & \sbest{95.6} & \sbest{95.1} \\
    & DnC     & \sbest{97.0} & 96.59 & \sbest{96.26} & \sbest{95.0} & 95.1 & 93.6 & 93.0 & 92.5 & 96.0 & 95.4 & 95.0 & 94.1 & 95.9 & 95.2 & 94.7 & 93.7 \\
    & DP2Guard   & \best{97.2} & \best{96.9} & \best{96.6} & \best{95.4} & \best{96.4} & \best{95.4} & \best{95.3} & \best{95.0} & \best{97.0} & \best{96.5} & \best{96.0} & \best{95.2}  & \best{97.0} & \best{96.5} & \best{96.0} & \best{95.7} \\
    \midrule

    \multirow{6}{*}{\textbf{Fashion-MNIST}}
    & FedAvg     &78.0 & 77.4 & 76.0 & 72.3 & 72.0 & 65.4 & 50.0 & 10.0  & 76.0 & 74.4 & 69.0 & 61.1  & 76.0 & 72.4 & 67.0 & 61.1  \\
    & FLTrust    & 79.2 & \sbest{79.0} & 78.5 & 78.2 & 79.2 & \sbest{79.0} & \sbest{78.5} & \sbest{74.7}   & 79.2 & \sbest{79.0} & \sbest{78.5} & 74.7  & 79.0 & \sbest{78.7} & 78.0 & 75.7 \\
    & MultiKrum  & 78.7 & 78.4 & 78.2 & 78.0  & 75.7 & 72.4 & 63.2 & 47.2  & 77.7 & 76.4 & 74.2 & 68.6 & 77.7 & 75.4 & 72.2 & 68.6 \\
    & ShieldFL   & 79.3 & 78.6 & 78.4 & 78.3 & \sbest{79.3} & 78.6 & 78.4 & 74.2   & \sbest{79.3} & 78.6 & 78.4 & \sbest{76.9}  & \sbest{79.3} & 78.6 & \sbest{78.4} & \sbest{76.9} \\
    & DnC        & \sbest{79.5} & \sbest{79.0} & \sbest{78.7} & \sbest{78.4}  & 79.2 & 77.2 & 76.7 & 73.9  & 79.2 & 78.2 & 76.7 & 74.1   & 78.2 & 77.0 & 75.7 & 74.4 \\
    & DP2Guard   & \best{79.9} & \best{79.5} & \best{79.2} & \best{78.7}  & \best{79.9} & \best{79.5} & \best{79.4} & \best{78.2} & \best{79.9} & \best{79.5} & \best{79.4} & \best{78.6}  & \best{79.4} & \best{78.9} & \best{78.7} & \best{78.3}\\
    \midrule

    \multirow{6}{*}{\textbf{CIFAR-10}}
      & FedAvg     & 65.0 & 62.4 & 58.0 & 50.3  & 58.0 & 47.4 & 28.0 & 10.0  &
      64.0 & 61.4 & 55.0 & 44.1  & 64.0 & 60.4 & 55.0 & 47.1 \\
      & FLTrust    & 72.5 & 72.0 & 71.5 & 70.2  & 72.5 & 71.0 & \sbest{70.5} & \sbest{68.7}  &
      72.2 & 71.0 & 70.5 & 68.7  & 72.0 & 71.7 & 71.0 & 69.7 \\
      & MultiKrum  & 71.0 & 70.4 & 69.2 & 67.0  & 68.1 & 62.8 & 52.2 & 38.3  &
      70.2 & 68.0 & 64.2 & 57.6  & 70.7 & 68.0 & 64.2 & 57.6 \\
      & ShieldFL   & 73.0 & 72.6 & \sbest{72.4} & 71.5  & \sbest{73.0} & \sbest{71.4} & 70.1 & 67.2  &
      \sbest{73.0} & \sbest{72.0} & \sbest{71.2} & \sbest{70.4}  & \sbest{73.3} & \sbest{72.6} & \sbest{72.0} & \sbest{70.9} \\
      & DnC        & \sbest{73.5} & \sbest{72.9} & \sbest{72.4} & \sbest{71.8}  & 71.1 & 69.6 & 69.0 & 66.5  &
      72.0 & 71.4 & 71.0 & 69.1  & 72.2 & 71.2 & 70.7 & 69.4 \\
      & DP2Guard   & \best{74.2} & \best{73.9} & \best{73.5} & \best{72.4}  & \best{73.4} & \best{72.5} & \best{72.3} & \best{71.0}  &
      \best{74.0} & \best{73.5} & \best{73.0} & \best{72.2}  & \best{74.0} & \best{73.5} & \best{73.0} & \best{72.7} \\

\bottomrule
\end{tabular}%
}
\end{table}

\textbf{Performance under Non-IID setting.} As shown in Table \ref{tab:def_per_noniid}, the Non-IID data distribution introduces additional challenges, with all methods experiencing accuracy reduction compared to the IID setting. Despite this, DP2Guard consistently maintains the best performance. On MNIST, DP2Guard achieves 93.5\% under LF attack, 92.5\% under Fang attack, 92.8\% under Min-Max attack, and 93.2\% under Min-Sum attack at 40\% adversary ratio, outperforming all baselines. The Fang attack proves most destructive in the Non-IID setting: FedAvg and MultiKrum nearly collapse on all three datasets, with accuracy dropping below 10\% and 24\% respectively on CIFAR-10 at 40\% adversary ratio. In contrast, DP2Guard retains 64.5\% accuracy under the same condition. On Fashion-MNIST and CIFAR-10, DP2Guard maintains a consistent advantage of 1\%--5\% over ShieldFL and DnC across all attack scenarios, demonstrating its effectiveness under data heterogeneity.

Overall, across all three datasets, four attack types, and both IID and Non-IID settings, DP2Guard consistently achieves the highest accuracy with the smallest performance degradation as the adversary ratio increases. These results validate the effectiveness of the hybrid detection mechanism and trust-based adaptive aggregation in DP2Guard, confirming its robustness against a wide range of poisoning threats in federated learning.

\begin{table}[H]
\centering
\caption{TABLE IV: Comparison of defense strategies against four poisoning attacks on MNIST, Fashion-MNIST, and CIFAR-10 in the Non-IID setting, with malicious-client ratios ranging from 0\% to 40\%.}
\label{tab:def_per_noniid}
\resizebox{\textwidth}{!}{%
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.35}
\begin{tabular}{ll cccc cccc cccc cccc}
\toprule
\multirow{2}{*}{\textbf{Data set}} & \multirow{2}{*}{\textbf{Method}}
& \multicolumn{4}{c}{\textbf{LF Attack}}
& \multicolumn{4}{c}{\textbf{Fang Attack}}
& \multicolumn{4}{c}{\textbf{Min-Max}}
& \multicolumn{4}{c}{\textbf{Min-Sum Attack}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}

&
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}
& \textbf{10} & \textbf{20} & \textbf{30} & \textbf{40}\\
\midrule

\multirow{6}{*}{\textbf{MNIST}}
  & FedAvg     & 91.2 & 88.4 & 83.0 & 76.3  & 84.0 & 72.2 & 42.4 & 10.0  &
  90.0 & 86.4 & 79.0 & 69.3  & 89.0 & 84.4 & 78.0 & 72.9 \\
  & FLTrust    & 94.5 & 94.0 & 93.5 & \sbest{92.2}  & \sbest{94.0} & 92.5 & 91.0 & \sbest{89.4}  &
  94.0 & 93.0 & 92.0 & 90.1  & 94.0 & 93.4 & 92.5 & 90.7 \\
  & MultiKrum  & 93.0 & 92.4 & 91.0 & 87.0  & 92.1 & 82.8 & 70.2 & 53.3  &
  93.0 & 90.0 & 86.0 & 74.5  & 92.7 & 88.0 & 83.0 & 74.3 \\
  & ShieldFL   & 95.0 & 94.5 & \sbest{93.8} & 91.5  & \sbest{94.0} & \sbest{93.0} & \sbest{91.5} & 88.0  &
  \sbest{95.0} & \sbest{94.0} & \sbest{93.0} & \sbest{91.4}  & \sbest{94.5} & \sbest{94.0} & \sbest{93.0} & \sbest{91.5} \\
  & DnC        & \sbest{95.2} & \sbest{94.6} & \sbest{93.8} & \sbest{92.0}  & 93.0 & 91.0 & 89.5 & 87.5  &
  94.0 & 93.4 & 92.5 & 90.1  & 93.5 & 92.8 & 91.7 & 89.7 \\
  & DP2Guard   & \best{95.5} & \best{95.2} & \best{94.8} & \best{93.5}  & \best{95.0} & \best{93.8} & \best{93.5} & \best{92.5}  &
  \best{95.2} & \best{94.5} & \best{94.0} & \best{92.8}  & \best{95.2} & \best{94.8} & \best{94.2} & \best{93.2} \\
  \midrule

  \multirow{6}{*}{\textbf{Fashion-MNIST}}
  & FedAvg     & 73.0 & 71.4 & 68.0 & 63.3  & 64.0 & 53.4 & 32.0 & 10.0  &
  71.0 & 67.4 & 60.0 & 50.1  & 71.0 & 65.4 & 58.0 & 50.1 \\
  & FLTrust    & 76.2 & 75.8 & 75.0 & 74.2  & 75.2 & 74.5 & 73.0 & \sbest{69.7}  &
  75.2 & 74.5 & 73.5 & 69.7  & 75.0 & 74.7 & 73.5 & 70.7 \\
  & MultiKrum  & 74.7 & 74.0 & 72.2 & 68.0  & 70.7 & 63.4 & 50.2 & 34.2  &
  73.7 & 70.4 & 65.2 & 56.6  & 73.7 & 69.4 & 63.2 & 56.6 \\
  & ShieldFL   & 76.3 & 75.6 & 75.0 & 74.3  & \sbest{75.3} & \sbest{74.6} & \sbest{73.4} & 69.2  &
  \sbest{76.0} & \sbest{75.0} & \sbest{74.0} & \sbest{72.4}  & \sbest{76.3} & \sbest{75.6} & \sbest{74.4} & \sbest{72.4} \\
  & DnC        & \sbest{76.5} & \sbest{76.0} & \sbest{75.2} & \sbest{74.4}  & 74.2 & 72.2 & 70.7 & 67.9  &
  75.2 & 74.0 & 72.2 & 69.1  & 74.2 & 73.0 & 71.0 & 69.4 \\
  & DP2Guard   & \best{77.0} & \best{76.5} & \best{76.2} & \best{75.4}  & \best{76.9} & \best{76.0} & \best{75.4} & \best{74.2}  &
  \best{76.9} & \best{76.5} & \best{75.9} & \best{74.6}  & \best{76.0} & \best{75.9} & \best{75.4} & \best{74.8} \\
  \midrule

  \multirow{6}{*}{\textbf{CIFAR-10}}
  & FedAvg     & 57.0 & 54.4 & 49.0 & 40.3  & 48.0 & 35.4 & 18.0 & 10.0  &
  56.0 & 53.4 & 46.0 & 34.1  & 56.0 & 52.4 & 46.0 & 37.1 \\
  & FLTrust    & 66.5 & 65.8 & 65.0 & 63.2  & 66.0 & 64.5 & 63.0 & \sbest{60.7}  &
  66.2 & 64.5 & 63.5 & 61.2  & 66.0 & 65.2 & 64.5 & 62.2 \\
  & MultiKrum  & 63.0 & 62.0 & 59.2 & 55.0  & 58.1 & 50.8 & 38.2 & 24.3  &
  62.2 & 58.0 & 52.2 & 43.6  & 62.7 & 58.0 & 52.2 & 43.6 \\
  & ShieldFL   & 67.3 & 66.6 & \sbest{66.0} & 64.5  & \sbest{67.0} & \sbest{65.0} & \sbest{63.1} & 59.2  &
  \sbest{67.0} & \sbest{66.0} & \sbest{64.8} & \sbest{63.4}  & \sbest{67.3} & \sbest{66.2} & \sbest{65.5} & \sbest{64.0} \\
  & DnC        & \sbest{67.5} & \sbest{66.9} & \sbest{66.0} & \sbest{65.0}  & 64.1 & 62.6 & 61.0 & 58.5  &
  66.0 & 65.0 & 64.2 & 62.1  & 66.2 & 65.0 & 64.0 & 62.4 \\
  & DP2Guard   & \best{68.5} & \best{68.0} & \best{67.5} & \best{66.4}  & \best{67.4} & \best{66.5} & \best{66.0} & \best{64.5}  &
  \best{68.0} & \best{67.5} & \best{67.0} & \best{65.7}  & \best{68.0} & \best{67.5} & \best{67.0} & \best{66.2} \\
\bottomrule
\end{tabular}%
}
\end{table}

\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C5}{
Table 3 presents the theoretical cost of DP2Guard; however, the authors merely describe the expenses of DP, SMPC, and HE as 'being substantial' without any theoretical or quantitative analysis to substantiate this claim.
}
\end{myquoteR2}
}

\resptotwo{R2.C5}{
We thank the reviewer for this suggestion. In the revised manuscript, we have addressed this in two ways.
First, we have added a theoretical complexity comparison in Table VI, which presents the computational and communication complexity of DP2Guard alongside HE-based schemes (PEFL and ShieldFL) and a SMPC-based scheme (VerifyNet) on both server and client sides. 
The analysis clearly shows that DP2Guard achieves the lowest client-side overhead, requiring only $\mathcal{O}\left(d T_{\text {prg }}\right)+\mathcal{O}\left(d T_{\text {add }}\right)$ computation compared to $\mathcal{O}\left(d T_{\text {phe }}\right)$ for HE-based schemes, where $T_{\text {phe }} \gg T_{\text {add }}$. Second, we have supplemented this with quantitative experimental results. Fig. 8 reports the actual per-round computation time and communication cost breakdown, and Fig. 9 evaluates the scalability under different numbers of clients. These results provide both theoretical and empirical evidence that DP2Guard incurs significantly lower overhead than HE-based and VSS-based alternatives. The updated analysis is presented in Section \ref{sec:complexity_analysis} of the revised manuscript.

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\captionsetup{labelformat=empty}
\caption{TABLE V: Comparison of computational and communication complexity.}
\label{tab:cost_analysis}
\begin{tabular}{lccccc}
\toprule
\textbf{Scheme} & \textbf{Technique} & \multicolumn{2}{c}{\textbf{Computation}} & \multicolumn{2}{c}{\textbf{Communication}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 & & \textbf{Server} & \textbf{Client} & \textbf{Server} & \textbf{Client} \\
\midrule
PEFL [37]
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
VerifyNet [19]
& VSS
& $\mathcal{O}(n^2 d T_{\text{vss}})$
& $\mathcal{O}(dN T_{\text{vss}})$
& $\mathcal{O}((n^2+nd)|\omega_{\text{vss}}|)$
& $\mathcal{O}((N+d)|\omega_{\text{vss}}|)$ \\
ShieldFL [36]
& PHE
& $\mathcal{O}(n^2 d T_{\text{phe}})$
& $\mathcal{O}(d T_{\text{phe}})$
& $\mathcal{O}(nd|\omega_{\text{phe}}|)$
& $\mathcal{O}(d|\omega_{\text{phe}}|)$ \\
DP2Guard
& GSM
& $\mathcal{O}(n^2 d T_{\text{add}})$
& $\mathcal{O}(d T_{\text{prg}}) + \mathcal{O}(d T_{\text{add}})$
& $\mathcal{O}(nd|\omega|)$
& $\mathcal{O}(2d|\omega|)$ \\
\bottomrule
\end{tabular}
\vspace{2pt}
\begin{tablenotes}
\footnotesize
\item PHE: partially homomorphic encryption; GSM: gradient splitting and masking; VSS: verifiable secret sharing. $d$: gradient dimension; $n$: number of clients. $T_{\text{prg}}$: cost of generating a pseudo-random number; $T_{\text{add}}$: cost of a plaintext addition; $T_{\text{phe}}$: cost of a PHE encryption ($T_{\text{phe}} \gg T_{\text{add}}$); $T_{\text{vss}}$: cost of generating a VSS share. $|\omega|$: size of a plaintext number; $|\omega_{\text{phe}}|$: size of a PHE ciphertext ($|\omega_{\text{phe}}| \gg |\omega|$); $|\omega_{\text{vss}}|$: size of a VSS share.
\end{tablenotes}
\end{table}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C6}{
In Section II, the authors note that DPFLA assumes non-colluding servers, thus vulnerable to collusion attacks. Doesn’t DP2Guard have the same weakness? Is the assumption that S1 and S2 are honest-but-curious yet non-colluding sufficiently realistic?
}
\end{myquoteR2}
}

\resptotwo{R2.C6}{
We appreciate the reviewer's comment. Although \dbname also relies on a non-collusion assumption, this assumption is strictly weaker than that of DPFLA and easier to satisfy in practice. Specifically, DPFLA requires the server not to collude with any of the potentially large number of participating clients, meaning that compromising even a single client suffices to break the assumption. In contrast, \dbname only assumes that two servers $S_1$ and $S_2$ do not collude with each other, significantly narrowing the attack surface from "server vs. any of N clients" to "server vs. one other server." 
Regarding the realism of this assumption, two-server non-collusion model is a standard and widely adopted assumption in secure multi-party computation and privacy-preserving machine learning. 
In practice, the two servers can be operated by independent entities.
For example, $S_1$ deployed on Amazon AWS and $S_2$ on Microsoft Azure, where the providers' competing commercial interests, contractual obligations, and reputational risks make collusion both unlikely and costly.
The non-collusion guarantee can be further strengthened through cross-jurisdictional deployment, third-party audits, and trusted execution environments (TEEs). 

To further validate this distinction empirically, we have conducted gradient inversion attack experiments under a server-client collusion scenario, comparing DP2Guard with DPFLA. As shown in Fig. 7, when a server colludes with a client, DPFLA fails to protect gradient privacy and the attacker can successfully reconstruct recognizable training images. Under the same collusion setting, DP2Guard maintains substantially degraded reconstruction quality insufficient for a successful attack, as DP2Guard does not rely on the non-collusion assumption between servers and clients. 

We have revised the manuscript to present the collusion attack experiments in Section \ref{sec:privacy_risk_evaluation}.

\begin{modificationR2}{}

To evaluate the privacy-preserving effectiveness of DP2Guard, we conduct gradient inversion attacks using the DLG (Deep Leakage from Gradients) [59] algorithm, which attempts to reconstruct private training data from observed gradients. Experiments are performed on both the MNIST and CIFAR-10 datasets.

We first compare DP2Guard with ShieldFL and FedAvg under the standard honest-but-curious server model. As shown in Fig. \ref{fig:gradient_inversion}, FedAvg, which provides no privacy protection, allows the attacker to successfully reconstruct recognizable training images. 
In contrast, both ShieldFL and DP2Guard effectively prevent gradient reconstruction, with the reconstructed images being indistinguishable from random noise. These results demonstrate that the lightweight gradient splitting and masking mechanism in DP2Guard provides privacy protection comparable to the HE-based approach adopted by ShieldFL.

We further evaluate the privacy resilience under a more challenging server-client collusion scenario, comparing DP2Guard with DPFLA. As shown in Fig. \ref{fig:gradient_inversion_collusion}, when a server colludes with a client, DPFLA fails to protect gradient privacy, and the attacker can successfully reconstruct recognizable training images. 
Under the same collusion setting, DP2Guard exhibits some residual visual features in the reconstructed images; however, the reconstruction quality is severely degraded and insufficient for a successful attack. 
This is because DP2Guard only requires non-collusion between the two servers $S_1$ and $S_2$, and does not rely on the assumption of non-collusion between servers and clients. 
These results confirm that DP2Guard provides stronger privacy protection than DPFLA even under server-client collusion.

\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/comparison_mnist.eps}
        \caption{MNIST dataset.}
        \label{fig:gradinv_noenc}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/comparison_cifar10.eps}
        \caption{CIFAR-10 dataset.}
        \label{fig:gradinv_paillier}
    \end{subfigure}
    \captionsetup{labelformat=empty}
    \caption{Fig. 6: Visual comparison of images reconstructed by the DLG attack under different defense mechanisms on MNIST and CIFAR-10 datasets.}
    \label{fig:gradient_inversion}
\end{figure}
\vspace{-10mm}
\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/collusion_mnist.eps}
        \caption{MNIST dataset.}
        \label{fig:gradinv_noenc}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/privacy/collusion_cifar10.eps}
        \caption{CIFAR-10 dataset.}
        \label{fig:gradinv_paillier}
    \end{subfigure}
    \captionsetup{labelformat=empty}
    \caption{Fig. 7: Visual comparison of images reconstructed by the DLG attack under server-client collusion between DPFLA and DP2Guard on MNIST and CIFAR-10 datasets.}
    \label{fig:gradient_inversion_collusion}
\end{figure}
\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C7}{
In the proof of Thm. 1, $\textbf{Hyb}_1$: and $\textbf{Hyb}_2$: claim that an attacker cannot distinguish a valid masked gradient share from a uniform random vector. However, in practice, an attacker could exploit meta-information such as packet receive timestamps (e.g., the two packets the attacker has eavesdropped were likely sent by client i to $S_1$ and $S_2$ at nearly the same time) to pair $\mathbf{g}_i^{(1)}$ and $\mathbf{g}_i^{(2)}$ and sum them. At the extreme, an attacker could brute-force all possible pairs of eavesdropped gradients and use those sums to try to infer private information. This casts doubt on whether the proposed random gradient splitting and masking can truly replace DP/SMPC/HE in realistic and general settings.
}
\end{myquoteR2}
}

\resptotwo{R2.C7}{
We appreciate the reviewer's comment. 
Under the semi-honest non-collusion server model adopted in \dbname, Theorem 1 rigorously proves that neither server can individually infer the original gradient from the masked share it receives, as each share is computationally indistinguishable from a uniformly random vector.
However, as the reviewer correctly points out, if a global external eavesdropper can simultaneously monitor both communication channels, it could potentially pair the two gradient shares via metadata such as timestamps and recover the original gradient by summing them. 
We acknowledge this as a limitation of the current design. 
In future work, we plan to enhance security by integrating lightweight homomorphic encryption or differential privacy techniques into the existing framework, ensuring that gradient shares remain protected even when paired and summed, thereby extending the security guarantee to stronger threat models while preserving low computational overhead.

We have revised Section \ref{sec:concludes} to discuss this limitation and the aforementioned future research directions.

\begin{modificationR2}{}
In this paper, we presented DP2Guard, a lightweight PPFL framework designed to address the dual challenges of privacy leakage and vulnerability to model poisoning. To reduce computational overhead, DP2Guard replaces traditional cryptographic techniques with an efficient gradient splitting and masking strategy that protects the privacy of local model updates. To improve robustness, we designed a hybrid anomaly detection mechanism that combines cosine similarity and spectral analysis to effectively identify malicious updates, complemented by a trust scoring mechanism that penalizes both excluded and surviving anomalous clients. Furthermore, blockchain is integrated to provide a secure and auditable training process. Extensive experimental results demonstrate that DP2Guard achieves superior performance compared to state-of-the-art defenses, offering enhanced robustness and lower communication and computation costs.

Despite these advantages, DP2Guard has certain limitations that warrant further investigation. First, the current gradient splitting and masking mechanism assumes that no global external eavesdropper can simultaneously monitor both communication channels. If such an eavesdropper exists and can bypass transport-layer encryption, it could potentially pair the two gradient shares and recover the original gradient. In future work, we plan to integrate lightweight homomorphic encryption or differential privacy techniques to ensure that gradient shares remain protected even when paired and summed. Second, under largescale partial participation settings with very low participation rates, the trust scores of inactive clients may not be updated frequently enough, reducing the effectiveness of the trust evaluation. We plan to address this by incorporating a trust score decay mechanism for inactive clients to maintain reliable trust evaluation under such scenarios.
\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C8}{
If EWMA updates the trust score as in Eq. (22), the EWMA coefficient (i.e., the training hyperparameter) $\beta$ will be important depending on the actual environment. What value of $\beta$ was used in each experimental setting?
}
\end{myquoteR2}
}

\resptotwo{R2.C8}{We would like to thank the reviewer for the valuable suggestion. To further investigate the impact of $\beta$ on performance, we have conducted a sensitivity analysis under different attack intensities in the revised manuscript. Fig. 10 (a) illustrates the convergence curves under different $\beta$ values with a 40\% Byzantine ratio on the MNIST dataset. A larger $\beta$ assigns excessive weight to historical trust, allowing malicious clients to maintain high trust scores over extended periods, resulting in slow convergence and limited accuracy. A smaller $\beta$ responds rapidly to current-round behavior but introduces excessive trust score fluctuations, leading to unstable aggregation. Fig. 10 (b) further demonstrates this finding across different Byzantine ratios, where all curves exhibit an inverted-U shape peaking at $\beta= 0.7$, which consistently achieves the best balance between responsiveness and stability. Based on these results, we adopt $\beta= 0.7$ as the default setting across all experiments. We have added this sensitivity analysis and the corresponding discussion in Section \ref{sec:sensitivity_analysis} of the revised manuscript.

\begin{modificationR2}{}
To investigate the sensitivity of DP2Guard to the parameter $\beta$, we conduct a parameter sensitivity analysis under different attack intensities. 
Fig. \ref{fig:beta_accuracy_rounds} illustrates the convergence curves under different $\beta$ values with a 40\% Byzantine ratio on the MNIST dataset. 
A larger $\beta$ (e.g., 0.9) assigns excessive weight to historical trust, allowing malicious clients to maintain high trust scores over extended periods, resulting in slow convergence and a final accuracy of only 70.2\%. 
A smaller $\beta$ (e.g., 0.1) responds rapidly to current-round behavior but introduces excessive trust score fluctuations, leading to unstable aggregation and a limited accuracy of 77.8\%. In contrast, $\beta = 0.7$ achieves the fastest convergence and the highest accuracy, effectively balancing responsiveness and stability. 
Fig. \ref{fig:beta_final_metrics} further demonstrates this finding across different byzantine ratios, where all curves exhibit an inverted-U shape peaking at $\beta = 0.74$. 
Based on these results, we adopt $\beta=0.7$ as the default setting across all experiments.

\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/sensitive_analysis/beta_convergence.png}
        \caption{Convergence with different $\beta$.}
        \label{fig:beta_accuracy_rounds}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{result/sensitive_analysis/beta_final.png}
        \caption{Effect of $\beta$ under varying Byzantine ratios.}
        \label{fig:beta_final_metrics}
    \end{subfigure}
    \caption{Fig. 10: Impact of the factor $\beta$ on CIFAR-10. (a) Test accuracy over communication rounds  with 40\% Byzantine clients for different  $\beta$. (b) Test accuracy versus  $\beta$ under different Byzantine client ratios.}
    \label{fig:sensitivity_analysis}
\end{figure}
\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C9}{
If EWMA updates the trust score as in Eq. (22), wouldn’t an attacker who arbitrarily turns the attack on and off each round substantially reduce the effectiveness of the scheme?
}
\end{myquoteR2}
}

\resptotwo{R2.C9}{
We appreciate the reviewer's comment. 
In our implementation, DP2Guard employs a two-layered defense mechanism against on-off attacks. 
The first layer is per-round anomaly detection, which serves as the primary defense. 
In each round, server $S_2$ independently performs spectral analysis, cosine similarity evaluation, and K-means clustering based on the feature vector $\mathbf{f}_i=[s_i, c_i]^{\top}$ to identify and exclude anomalous gradients. 
This detection is executed independently of historical trust scores, meaning that even if an on-off attacker has accumulated a high trust score during benign rounds, its malicious gradient will still be detected and excluded in the attack round. 
The second layer is the EWMA trust score, which is updated for all clients in every round, including those excluded by clustering. 
Since excluded clients have been assigned to the anomalous cluster, their feature vectors are far from the benign cluster centroid $\boldsymbol{\mu}^{(t)}$, resulting in a large Dis $_i^{(t)}$ and a near-zero $\gamma_i^{(t)}$, which causes their trust score to drop significantly. 
Consequently, when the attacker returns to a benign round and passes the clustering detection, its accumulated trust score remains lower than that of consistently honest clients, resulting in a smaller aggregation weight $\tau_i^{(t)}$. 
Therefore, per-round detection and trust penalization together mitigate on-off attacks from both exclusion and weight reduction perspectives.

We have clarified this in Section \ref{sec:design} of the revised manuscript.

\begin{modificationR2}{}
4) Trust Scoring-Based Weight Computation: The trust scoring mechanism ensures that individual client nodes contribute appropriately to the global model aggregation process [52]. Unlike prior approaches that rely solely on per-round behavior, DP2Guard introduces a time-evolving trust evaluation scheme that captures clients' long-term reliability.

In each round $t$, server $\mathcal{S}_2$ calculates the Euclidean distance between each client's feature vector $\mathbf{f}_i^{(t)}$ and the benign cluster centroid $\boldsymbol{\mu}^{(t)}$:
\begin{equation}
    \operatorname{Dis}_i^{(t)}=\left\|\mathbf{f}_i^{(t)}-\boldsymbol{\mu}^{(t)}\right\|
\end{equation}
Based on this distance, the direct trust score for device $E_i$ is computed as:
\begin{equation}
    \gamma_i^{(t)}=1 /\left(1+\operatorname{Dis}_i^{(t)}\right)
\end{equation}
For clients in the benign cluster, their feature vectors are close to the centroid, resulting in a small $\mathrm{Dis}_i{ }^{(t)}$ and a high $\gamma_i^{(t)}$. For clients assigned to the anomalous cluster, their feature vectors are far from the benign centroid, leading to a large $\operatorname{Dis}_i^{(t)}$ and a near-zero $\gamma_i^{(t)}$.

To balance historical performance and recent behavior, DP2Guard utilizes a time-based trust mechanism. For each client $i$, the trust score is updated as:
\begin{equation}
    \operatorname{Trust}_i^{(t)}=\beta \cdot \operatorname{Trust}_i^{(t-1)}+(1-\beta) \cdot \gamma_i^{(t)}, \quad \beta \in[0,1)
\end{equation}
Note that this update is applied to all clients in each round, including those excluded by the clustering mechanism. For excluded clients, their near-zero $\gamma_i^{(t)}$ causes a significant drop in their trust score, ensuring that clients exhibiting malicious behavior are penalized even when their gradients are already excluded from aggregation. This is particularly effective against on-off attacks where adversaries alternate between benign and malicious behavior.
The normalized trust value is used to compute the aggregation weight:
$$
\tau_i^{(t)}=\frac{\operatorname{Trust}_i^{(t)}}{\sum_{j=1}^N \operatorname{Trust}_j^{(t)}}
$$
Server $\mathcal{S}_2$ then applies these weights to aggregate the received masked gradients:
\begin{equation}
    \tilde{\mathbf{g}}_{\text {agg }}^{(2)}=\sum_{i=1}^N \tau_i^{(t)} \cdot \tilde{\mathbf{g}}_i^{(2)}
\end{equation}
Then, both $\tilde{\mathbf{g}}_{\text {agg }}^{(2)}$ and trust weights $\left\{\tau_i^{(t)}\right\}_{i=1}^N$ are published to the blockchain. 
\end{modificationR2}
}

\ifthenelse{\boolean{showquestion}}{
\begin{myquoteR2}
\rcomment{R2.C10}{
If EWMA updates the trust score as in Eq. (22), wouldn’t a sparse update of trust scores—especially when the number of clients is large, so that only a subset of clients participates in each round—reduce the usefulness of the trust score?
}
\end{myquoteR2}
}

\resptotwo{R2.C10}{
We appreciate the reviewer's comment. 
To investigate the impact of partial participation on the trust mechanism, we have conducted experiments under different client scales $N \in\{200,500,1000,1500,2000\}$ and participation rates $\{10 \%, 20 \%, 40 \%, 60 \%, 80 \%, 100 \%\}$ on the MNIST dataset under the Fang attack with $40 \%$ adversary ratio. As shown in Fig. 11, when the participation rate is above $40 \%$, DP2Guard maintains stable accuracy above $92 \%$ across all client scales, with degradation within $3\%$ compared to full participation. When the participation rate drops to $20 \%$, larger client scales ( $N \geq 1000$ ) still achieve above $90 \%$ accuracy. However, when the participation rate falls below $20 \%$, performance degrades noticeably across all scales, particularly for smaller $N$ where $N=200$ at 10\% participation drops to approximately $681 \%$. This indicates that at very low participation rates, the trust scores are insufficiently updated per round, limiting the effectiveness of the EWMA-based trust evaluation. In future work, we plan to address this limitation by incorporating a trust score decay mechanism for inactive clients to maintain the reliability of trust evaluation under very low participation rates. 

We have discussion in Section \ref{sec:concludes} of the revised manuscript.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.33\columnwidth]{result/accuracy_participation.png}
    \caption{Fig. 11 Accuracy under different participation rates and client scales.}
    \label{fig:beta_accuracy_rounds}
\end{figure}
\begin{modificationR2}{}
In this paper, we presented DP2Guard, a lightweight PPFL framework designed to address the dual challenges of privacy leakage and vulnerability to model poisoning. To reduce computational overhead, DP2Guard replaces traditional cryptographic techniques with an efficient gradient splitting and masking strategy that protects the privacy of local model updates. To improve robustness, we designed a hybrid anomaly detection mechanism that combines cosine similarity and spectral analysis to effectively identify malicious updates, complemented by a trust scoring mechanism that penalizes both excluded and surviving anomalous clients. Furthermore, blockchain is integrated to provide a secure and auditable training process. Extensive experimental results demonstrate that DP2Guard achieves superior performance compared to state-of-the-art defenses, offering enhanced robustness and lower communication and computation costs.

Despite these advantages, DP2Guard has certain limitations that warrant further investigation. First, the current gradient splitting and masking mechanism assumes that no global external eavesdropper can simultaneously monitor both communication channels. If such an eavesdropper exists and can bypass transport-layer encryption, it could potentially pair the two gradient shares and recover the original gradient. In future work, we plan to integrate lightweight homomorphic encryption or differential privacy techniques to ensure that gradient shares remain protected even when paired and summed. Second, under largescale partial participation settings with very low participation rates, the trust scores of inactive clients may not be updated frequently enough, reducing the effectiveness of the trust evaluation. We plan to address this by incorporating a trust score decay mechanism for inactive clients to maintain reliable trust evaluation under such scenarios.
\end{modificationR2}

}


\setcounter{page}{0}
\setcounter{section}{0}
\setcounter{figure}{0}

